Mozart: A Chiplet Ecosystem-Accelerator Codesign Framework for Composable Bespoke Application Specific Integrated Circuits

Modern AI acceleration faces a fundamental challenge: conventional assumptions about memory requirements, batching effectiveness, and latency-throughput tradeoffs are systemwide generalizations that ignore the heterogeneous computational patterns of individual neural network operators. However, going towards network-level customization and operator-level heterogeneity incur substantial Non-Recurring Engineering (NRE) costs. While chiplet-based approaches have been proposed to amortize NRE costs, reuse opportunities remain limited without carefully identifying which chiplets are truly necessary. This paper introduces Mozart, a chiplet ecosystem and accelerator codesign framework that systematically constructs low cost bespoke application-specific integrated circuits (BASICs). BASICs leverage operator-level disaggregation to explore chiplet and memory heterogeneity, tensor fusion, and tensor parallelism, with place-and-route validation ensuring physical implementability. The framework also enables constraint-aware system-level optimization across deployment contexts ranging from datacenter inference serving to edge computing in autonomous vehicles. The evaluation confirms that with just 8 strategically selected chiplets, Mozart-generated composite BASICs achieve 43.5%, 25.4%, 67.7%, and 78.8% reductions in energy, energy-cost product, energy-delay product (EDP), and energy-delay-cost product compared to traditional homogeneous accelerators. For datacenter LLM serving, Mozart achieves 15-19% energy reduction and 35-39% energy-cost improvement. In speculative decoding, Mozart delivers throughput improvements of 24.6-58.6% while reducing energy consumption by 38.6-45.6%. For autonomous vehicle perception, Mozart reduces energy-cost by 25.54% and energy by 10.53% under real-time constraints.

==> case_studies/stable_diffusion.tex <==
This case study demonstrates Mozart's effectiveness on hybrid generative models that combine multiple computational paradigms within a single inference pipeline. Stable Diffusion exemplifies the architectural diversity challenge identified in our introduction, incorporating convolutional layers, attention mechanisms, and specialized normalization operations that exhibit fundamentally different computational characteristics.

Stable Diffusion's multi-stage pipeline validates all five operator-level insights from Section~\ref{sec:motivation}. The model combines U-Net architectures with cross-attention mechanisms and varies computational intensity across diffusion timesteps, creating a complex optimization landscape that exposes the limitations of homogeneous acceleration approaches.

\paragraph{Hybrid Architecture Challenges}
Generative diffusion models present unique operator-level challenges that Mozart's framework is designed to address:

\begin{itemize}
    \item \textbf{Cross-attention operations} require high memory bandwidth (Insight 1) but benefit from specialized attention accelerator designs (Insight 4)
    \item \textbf{Convolutional layers} exhibit spatial data reuse patterns that conflict with attention mechanisms' access patterns
    \item \textbf{Timestep-dependent computation} creates dynamic workload characteristics where batching effectiveness varies across pipeline stages (Insight 2)
    \item \textbf{Multi-resolution processing} in the U-Net architecture creates heterogeneous memory requirements across scales
\end{itemize}

Mozart addresses these challenges through operator-level chiplet allocation: attention blocks execute on high-bandwidth specialized chiplets, convolutional operations utilize spatial-locality-optimized designs, and normalization layers leverage compute-efficient implementations.

\paragraph{Generative Model Optimization}
Unlike discriminative models with fixed computational patterns, generative models like Stable Diffusion exhibit time-varying computational requirements across diffusion steps. Early timesteps require more computational resources while later steps focus on refinement, creating opportunities for dynamic resource allocation that validate Insight 3's operator-dependent latency-throughput tradeoffs.

We compare Mozart's heterogeneous approach against:
\begin{itemize}
    \item \textbf{GPU baseline}: General-purpose acceleration across all operators
    \item \textbf{Homogeneous \gls{mcm}}: Single chiplet design handling diverse operator requirements
    \item \textbf{Mozart heterogeneous \gls{mcm}}: Operator-specific chiplet allocation with dynamic resource scheduling
\end{itemize}

Evaluation metrics include generation quality (FID scores), energy efficiency per generated image, and throughput under quality constraints, demonstrating Mozart's effectiveness across the full spectrum of generative AI deployment scenarios.
